ARS: Automatic Routing Solver with Large Language Models

Real-world Vehicle Routing Problems (VRPs) are characterized by a variety of practical constraints, making manual solver design both knowledge-intensive and time-consuming. Although there is increasing interest in automating the design of routing algorithms, existing research has explored only a limited array of VRP variants and fails to adequately address the complex and prevalent constraints encountered in real-world situations. To fill this gap, this paper introduces RoutBench, a benchmark of 1,000 VRP variants derived from 24 attributes, for evaluating the effectiveness of automatic routing solvers in addressing complex constraints. Along with RoutBench, we present the Automatic Routing Solver (ARS), which employs Large Language Model (LLM) agents to enhance a backbone algorithm framework by automatically generating constraint-aware heuristic code, based on problem descriptions and several representative constraints selected from a database. Our experiments show that ARS outperforms state-of-the-art LLM-based methods and commonly used solvers, automatically solving 91.67% of common VRPs and achieving at least a 30% improvement across all benchmarks.

==> Base-model/Base.tex <==
def check_constraints(solution: VrpState) -> bool:
  """
  Check if the solution satisfies the constraints.

  Args:
    solution (VrpState): An object representing the VRP solution.
      - problem_data (dict): A dictionary with problem details:
        - "demand": A 1D NumPy array of node demands (0 for the depot).
        - "capacity": Maximum load capacity per vehicle.
        - "edge_weight": A 2D NumPy array of node distances.
        - "service_time": A 1D NumPy array of node service times (0 for the depot).
        - "time_window": A list of [earliest start, latest end] time windows for servicing each node.
      - routes (list): A list of routes, where each route is a list of node IDs (integers, excluding the depot node 0).

==> Base-model/Base1.tex <==
  Return:
    bool: True if the solution satisfies the constraints, False otherwise.

  Note:
    The above "Args" cannot be added or modified, and no data outside the "solution" object should be used or added.
  """
  # Your code goes here...

  return True

==> Base-model/CVRP.tex <==
def check_constraints(solution: VrpState) -> bool:
  """
  Check if the solution satisfies the constraints.

  Args:
    solution (VrpState): An object representing the VRP solution.
      - problem_data (dict): A dictionary with problem details:
        - "edge_weight": A 2D NumPy array of node distances.
        - "demand": A 1D NumPy array of node demands (0 for the depot).
        - "capacity": Maximum load capacity per vehicle.
      - routes (list): A list of routes, where each route is a list of node IDs (integers, excluding the depot node 0).

  Return:
    bool: True if the solution satisfies the constraints, False otherwise.

  Note:
    The above "Args" cannot be added or modified, and no data outside the "solution" object should be used or added.
  """
  for route in solution.routes:
    total_demand = sum(solution.problem_data["demand"][node] for node in route)
    if total_demand > solution.problem_data["capacity"]:
      return False
  return True


==> Base-model/PVRP.tex <==
def check_constraints(solution: VrpState) -> bool:
  """
  Check if the solution satisfies the constraints.

  Args:
    solution (VrpState): An object representing the VRP solution.
      - problem_data (dict): A dictionary with problem details:
        - "edge_weight": A 2D NumPy array of node distances.
      - routes (list): A list of routes, where each route is a list of node IDs (integers, excluding the depot node 0).

  Return:
    bool: True if the solution satisfies the constraints, False otherwise.

  Note:
    The above "Args" cannot be added or modified, and no data outside the "solution" object should be used or added.
  """
  # Define priority levels for nodes. Higher numbers mean higher priority.
  priority_levels = {
    17: 1,  # Priority level 1 (highest priority)
    19: 1,  # Priority level 1 (highest priority)
  }
  
  # Default priority for non-listed nodes (lowest priority)
  default_priority = 0

  for route in solution.routes:
    last_priority = max(priority_levels.values())  # Initialize to the highest priority

    for node in route:
      # Get current node's priority, using the default if not specified
      current_priority = priority_levels.get(node, default_priority)

      # If we encounter a node with higher priority than the last, the constraint is violated
      if current_priority > last_priority:
        return False

      # Update the last seen priority
      last_priority = current_priority

  return True


==> Base-model/VRPL.tex <==
def check_constraints(solution: VrpState) -> bool:
  """
  Check if the solution satisfies the constraints.

  Args:
    solution (VrpState): An object representing the VRP solution.
      - problem_data (dict): A dictionary with problem details:
        - "edge_weight": A 2D NumPy array of node distances.
      - routes (list): A list of routes, where each route is a list of node IDs (integers, excluding the depot node 0).

  Return:
    bool: True if the solution satisfies the constraints, False otherwise.

  Note:
    The above "Args" cannot be added or modified, and no data outside the "solution" object should be used or added.
  """
  max_route_length = 100
  distances = solution.problem_data["edge_weight"]

  for route in solution.routes:
    tour = [0] + route + [0]  # Add depot at the beginning and end of the route
    route_length = sum(distances[tour[idx - 1]][tour[idx]] for idx in range(1, len(tour)))

    # Check if the route length exceeds the maximum allowed length
    if route_length > max_route_length:
      return False

  return True


==> Base-model/VRPMPD.tex <==
def check_constraints(solution: VrpState) -> bool:
  """
  Check if the solution satisfies the constraints.

  Args:
    solution (VrpState): An object representing the VRP solution.
      - problem_data (dict): A dictionary with problem details:
        - "edge_weight": A 2D NumPy array of node distances.
        - "demand": A 1D NumPy array of node demands (0 for the depot).
        - "capacity": Maximum load capacity per vehicle.
      - routes (list): A list of routes, where each route is a list of node IDs (integers, excluding the depot node 0).

  Return:
    bool: True if the solution satisfies the constraints, False otherwise.

  Note:
    The above "Args" cannot be added or modified, and no data outside the "solution" object should be used or added.
  """
  pickup_nodes = {24: 10}  # Values in user requirements
  vehicle_capacity = solution.problem_data["capacity"]

  for route in solution.routes:
    current_load = 0

    for node in route:
      demand = solution.problem_data["demand"][node]

      if node in pickup_nodes:
        current_load -= pickup_nodes[node]  # When a pickup node is visited
      else:
        current_load += demand  # If not a pickup point, it must satisfy the vehicle capacity.

      # Check if the vehicle capacity is exceeded or negative after visiting this node
      if current_load > vehicle_capacity or current_load < 0:
        return False

  return True


==> Base-model/VRPS.tex <==
def check_constraints(solution: VrpState) -> bool:
  """
  Check if the solution satisfies the constraints.

  Args:
    solution (VrpState): An object representing the VRP solution.
      - problem_data (dict): A dictionary with problem details:
        - "edge_weight": A 2D NumPy array of node distances.
      - routes (list): A list of routes, where each route is a list of node IDs (integers, excluding the depot node 0).

  Return:
    bool: True if the solution satisfies the constraints, False otherwise.

  Note:
    The above "Args" cannot be added or modified, and no data outside the "solution" object should be used or added.
  """
  for route in solution.routes:
    if 1 in route and 10 in route:
      break
  else:
    # If no route contains both nodes 1 and 10
    return False

  return True


==> Base-model/VRPTW.tex <==
def check_constraints(solution: VrpState) -> bool:
  """
  Check if the solution satisfies the constraints.

  Args:
    solution (VrpState): An object representing the VRP solution.
      - problem_data (dict): A dictionary with problem details:
        - "edge_weight": A 2D NumPy array of node distances.
        - "service_time": A 1D NumPy array of node service times (0 for the depot).
        - "time_window": A list of [earliest start, latest end] time windows for servicing each node.
      - routes (list): A list of routes, where each route is a list of node IDs (integers, excluding the depot node 0).

  Return:
    bool: True if the solution satisfies the constraints, False otherwise.

  Note:
    The above "Args" cannot be added or modified, and no data outside the "solution" object should be used or added.
  """ 
  for route in solution.routes:
    current_time = 0  # Start at time 0
    tour = [0] + route + [0]  # Add depot at the beginning and end of the route

    for idx in range(1, len(tour)):
      arrive_time = current_time + solution.problem_data["edge_weight"][tour[idx - 1]][tour[idx]]
      wait_time = max(0, solution.problem_data["time_window"][tour[idx]][0] - arrive_time) 
      current_time = arrive_time + wait_time

      tw_start, tw_end = solution.problem_data["time_window"][tour[idx]]
      if current_time > tw_end:
        return False

      # Add the service time for the current node after arriving and waiting
      current_time += solution.problem_data["service_time"][tour[idx]]

  return True


==> Base-model/solver-result-CVRPTW/CPLEX1.tex <==
from docplex.mp.model import Model

def find_feasible_routes(solution: VrpState) -> list[list[int]]:
  """
  Finds feasible routes for a CVRPTW using CPLEX/DOcplex.

  Args:
    solution (VrpState): Contains problem_data dict with keys:
      - "capacity": Q
      - "demand": 1D numpy array, demand[0]=0
      - "edge_weight": 2D distance matrix
      - "time_window": time window, time_window[i]=(earliest, latest)
      - "service_time": service time for each node
      - optionally "num_vehicles": K
  Returns:
    List of routes (each a list of customer indices, excluding depot 0).
  """
  data = solution.problem_data
  Q = data["capacity"]
  demand = data["demand"]
  edge_weight = data["edge_weight"]
  time_window = data["time_window"]
  service_time = data["service_time"]
  num_nodes = len(demand)
  V = list(range(num_nodes))
  N = V[1:]
  K = data.get("num_vehicles", None)

  # Get the earliest and latest times for time windows
  earliest = {{i: time_window[i][0] for i in V}}
  latest = {{i: time_window[i][1] for i in V}}

  # Calculate a large number M as the upper bound for time constraints
  M = sum(latest[i] + service_time[i] + max(edge_weight[i]) for i in V)

  # Build model
  model = Model(name="VRPTW")
  model.parameters.timelimit = {run_time}  # Set time limit for solving

  # Decision variables x[i,j]
  arcs = [(i, j) for i in V for j in V if i != j]
  x = model.binary_var_dict(arcs, name="x")

  # MTZ load variables u[i] with lb=demand[i], ub=Q
  u = model.continuous_var_dict(
    N,
    lb={{i: float(demand[i]) for i in N}},
    ub=Q,
    name="u"
  )

==> Base-model/solver-result-CVRPTW/CPLEX2.tex <==
  # Time variables: arrival time at node i
  t = model.continuous_var_dict(V, lb=0, name="t")

  # Objective: minimize total distance
  model.minimize(model.sum(edge_weight[i, j] * x[i, j] for i, j in arcs))

  # Degree constraints: each customer exactly one in and one out
  for i in N:
    model.add_constraint(model.sum(x[i, j] for j in V if j != i) == 1)
    model.add_constraint(model.sum(x[j, i] for j in V if j != i) == 1)

  # Vehicle count limit at depot
  if K is not None:
    model.add_constraint(model.sum(x[0, j] for j in N) <= K)
    model.add_constraint(model.sum(x[i, 0] for i in N) <= K)

  # MTZ sub-tour elimination / capacity constraints
  for i, j in arcs:
    if i != 0 and j != 0:
      model.add_constraint(u[i] + demand[j] <= u[j] + Q * (1 - x[i, j]))

  # Time window constraints
  # Enforce time window ranges
  for i in V:
    model.add_constraint(earliest[i] <= t[i])
    model.add_constraint(t[i] <= latest[i])

  # Ensure time logic along the route is correct
  for i, j in arcs:
    if j != 0:  # No need to consider time window for returning to the depot
      model.add_constraint(
        t[i] + service_time[i] + edge_weight[i, j] <= t[j] + M * (1 - x[i, j])
      )

  # Solve
  sol = model.solve(log_output=True)
  if sol is None:
    logger.error("No solution found.")
    return []

  # Extract used arcs
  used = [(i, j) for (i, j) in arcs if x[i, j].solution_value > 0.5]

  # Build successor map
  succ = {{i: j for i, j in used}}

  # Reconstruct routes from depot
  routes = []
  starts = [j for i, j in used if i == 0]
  for st in starts:
    route = []
    cur = st
    while cur != 0:
      route.append(cur)
      cur = succ.get(cur, 0)
    routes.append(route)

  return routes

==> Base-model/solver-result-CVRPTW/Gurobi1.tex <==
from gurobipy import Model, GRB, quicksum
from typing import List

def find_feasible_routes(solution: VrpState) -> List[List[int]]:
  """
  Finds feasible routes for a CVRPTW using an optimization solver.

  Args:
    solution (VrpState): An object representing the VRP solution.
      - problem_data (dict): A dictionary with problem details:
         - "demand": A 1D NumPy array of node demands (0 for the depot).
         - "vehicles": Maximum vehicle.
         - "capacity": Maximum load capacity per vehicle.
         - "edge_weight": A 2D NumPy array or matrix of distances between nodes.

  Return:
    routes (list): A list of optimized routes, where each route is a list of node IDs (integers, excluding the depot node 0).
  """
  data = solution.problem_data
  num_nodes = len(data["demand"])
  demand = data["demand"]
  capacity = data["capacity"]
  vehicles = data["vehicles"]
  edge_weight = data["edge_weight"]
  service_time = data["service_time"]
  time_window = data["time_window"]

  model = Model("CVRPTW_PathLength")
  model.setParam('TimeLimit', 50)

  # Decision Variables
  x = model.addVars(num_nodes, num_nodes, vtype=GRB.BINARY, name="x")
  u = model.addVars(num_nodes, vtype=GRB.CONTINUOUS, name="u")  # For capacity
  arrival_time = model.addVars(num_nodes, vtype=GRB.CONTINUOUS, lb=0, name="arrival_time")

  # Objective: Minimize total distance
  model.setObjective(
    quicksum(edge_weight[i][j] * x[i, j] for i in range(num_nodes) for j in range(num_nodes) if i != j),
    GRB.MINIMIZE
  )

  # Core Constraints
  model.addConstrs((quicksum(x[i, j] for i in range(num_nodes) if i != j) == 1 for j in range(1, num_nodes)),
                   "in_degree")
  model.addConstrs((quicksum(x[i, j] for j in range(num_nodes) if i != j) == 1 for i in range(1, num_nodes)),
                   "out_degree")


==> Base-model/solver-result-CVRPTW/Gurobi2.tex <==
  model.addConstr(quicksum(x[0, j] for j in range(1, num_nodes)) <= vehicles, "max_vehicles")
  model.addConstr(quicksum(x[0, j] for j in range(1, num_nodes)) == quicksum(x[j, 0] for j in range(1, num_nodes)),
                  "depot_flow")
                  
  # MTZ Capacity Constraints
  model.addConstr(u[0] == 0, "u_depot")
  for j in range(1, num_nodes):
    model.addConstr(u[j] >= demand[j], f"u_min_{j}")
    model.addConstr(u[j] <= capacity, f"u_max_{j}")
    for i in range(num_nodes):
      if i != j:
        model.addConstr(
          u[j] >= u[i] + demand[j] - capacity * (1 - x[i, j]),
          f"mtz_cap_{i}_{j}"
        )

  # Time window constraints
  model.addConstr(arrival_time[0] == 0, name="StartTimeDepot")
  model.addConstrs(
    (arrival_time[i] + service_time[i] + edge_weight[i][j] <= arrival_time[j] + (1 - x[i, j]) * 1e6
     for i in range(num_nodes) for j in range(1, num_nodes) if i != j), name="TravelTime")
  model.addConstrs((arrival_time[j] >= time_window[j][0] for j in range(1, num_nodes)), name="EarliestArrival")
  model.addConstrs((arrival_time[j] <= time_window[j][1] for j in range(num_nodes)), name="LatestArrival")

  # Solve
  model.optimize()

  # Core route extraction logic
  routes = []
  if hasattr(model, 'status') and model.status in [GRB.OPTIMAL, GRB.TIME_LIMIT]:
    visited = set()
    for j in range(1, num_nodes):  # Skip depot
      if x[0, j].x > 0.5 and j not in visited:
        current, route = j, []
        while current != 0:  # Until return to depot
          route.append(current)
          visited.add(current)
          current = next((k for k in range(num_nodes) if k != current and x[current, k].x > 0.5), 0)
        if route:
          routes.append(route)
  return routes


==> Base-model/solver-result-CVRPTW/OR-tools1.tex <==
def find_feasible_routes(solution: VrpState) -> list[list[int]]:
  """
  Finds feasible routes for a VRP problem using an optimization solver.

  Args:
    solution (VrpState): An object representing the VRP solution.
      - problem_data (dict): A dictionary with problem details:
        - "capacity": Maximum load capacity per vehicle.
        - "demand": 1D numpy array, demand [0]=0.
        - "time_window": A 2D NumPy array where each row represents the [earliest, latest] time windows for servicing each node.
        - "service_time": service time for each node.
        - "edge_weight": 2D distance matrix.
  Return:
    routes (list): A list of optimized routes, where each route is a list of node IDs (integers, excluding the depot node 0).

  Note:
    The above "Args" cannot be added or modified, and no data outside the "solution" object should be used or added.
    Ensure each node is visited exactly once.
  """
  # Data Preprocessing
  data = solution.problem_data
  # Ensure all data types are correct
  edge_weight = data['edge_weight'].astype(np.int64)
  demands = [int(x) for x in data['demand'].astype(np.int64)]
  time_windows = [[int(tw[0]), int(tw[1])] for tw in data['time_window']]
  service_times = [int(st) for st in data['service_time'].astype(np.int64)]
  vehicle_capacity = int(data['capacity'])
  num_nodes = len(data["demand"])
  num_vehicles = num_nodes - 1

  # Create the routing index manager
  manager = pywrapcp.RoutingIndexManager(num_nodes, num_vehicles, 0)
  # Create Routing Model
  routing = pywrapcp.RoutingModel(manager)

  # Create and register a transit callback for distance.
  def distance_callback(from_index, to_index):
    # Returns the distance between the two nodes.
    from_node = manager.IndexToNode(from_index)
    to_node = manager.IndexToNode(to_index)
    return edge_weight[from_node][to_node]

  transit_callback_index = routing.RegisterTransitCallback(distance_callback)
  
  # Define cost of each arc.
  routing.SetArcCostEvaluatorOfAllVehicles(transit_callback_index)
  
  # Add Capacity constraint
  def demand_callback(from_index):

==> Base-model/solver-result-CVRPTW/OR-tools2.tex <==
    # Returns the demand of the node.
    from_node = manager.IndexToNode(from_index)
    return demands[from_node]
    
  demand_callback_index = routing.RegisterUnaryTransitCallback(demand_callback)
  routing.AddDimensionWithVehicleCapacity(
    demand_callback_index, 0, [vehicle_capacity] * num_vehicles, True, 'Capacity'
  )

  # Add Time Window constraint
  def time_callback(from_index, to_index):
    # Returns the travel time between the two nodes (excluding service time).
    from_node = manager.IndexToNode(from_index)
    to_node = manager.IndexToNode(to_index)
    return edge_weight[from_node][to_node]  # Only travel time, no service time

  time_callback_index = routing.RegisterTransitCallback(time_callback)
  horizon = time_windows[0][1]  # Maximum time limit for routes (depot's latest end time)
  routing.AddDimension(
    time_callback_index, horizon, horizon, False, 'Time'
  )

  # Set time windows for all nodes (including the depot)
  time_dimension = routing.GetDimensionOrDie('Time')
  for node_index in range(num_nodes):  # Include depot node
    index = manager.NodeToIndex(node_index)
    time_dimension.CumulVar(index).SetRange(time_windows[node_index][0], time_windows[node_index][1])
    # Add service time to the departure time
    routing.solver().Add(
      time_dimension.CumulVar(index) + service_times[node_index] <= time_dimension.CumulVar(index) + service_times[node_index]
    )

  # Solver Configuration
  search_params = pywrapcp.DefaultRoutingSearchParameters()
  search_params.first_solution_strategy = (
    routing_enums_pb2.FirstSolutionStrategy.PATH_CHEAPEST_ARC
  )
  search_params.time_limit.seconds = 50  # Timeout protection
  # Route Extraction
  routes = []
  if (result := routing.SolveWithParameters(search_params)):
    for vehicle_id in range(routing.vehicles()):
      index = routing.Start(vehicle_id)
    
      route = []
      while not routing.IsEnd(index):
        node = manager.IndexToNode(index)
        if node != 0:  # Filter out depot node
          route.append(node)
        index = result.Value(routing.NextVar(index))
      if route:  # Filter out empty routes
        routes.append(route)
        
  return routes

==> Base-model/solver-result-CVRPTW/Our_solver.tex <==
def check_constraints(solution: VrpState) -> bool:
  """
  Args:
    solution (VrpState): An object representing the VRP solution.
      - problem_data (dict): A dictionary with problem details:
         - "edge_weight": A 2D NumPy array of node distances.
         - "demand": A 1D NumPy array of node demands (0 for the depot).
         - "capacity": Maximum load capacity per vehicle.
         - "service_time": A 1D NumPy array of node service times (0 for the depot).
         - "time_window": A list of [earliest start, latest end] time windows for servicing each node.
      - routes (list): A list of routes, where each route is a list of node IDs (integers, excluding the depot node 0).

  Return:
    bool: True if the solution satisfies the constraints, False otherwise.

  Note:
    The above "Args" cannot be added or modified, and no data outside the "solution" object should be used or added.
  """
  for route in solution.routes:
    # Check Vehicle Capacity Constraint
    total_demand = sum(solution.problem_data["demand"][node] for node in route)
    if total_demand > solution.problem_data["capacity"]:
      return False

    # Check Time Windows Constraint
    current_time = 0  # Start at time 0
    tour = [0] + route + [0]  # Add depot at the beginning and end of the route

    for idx in range(1, len(tour)):
      arrive_time = current_time + solution.problem_data['edge_weight'][tour[idx - 1]][tour[idx]]
      wait_time = max(0, solution.problem_data['time_window'][tour[idx]][0] - arrive_time)  # Wait if early
      current_time = arrive_time + wait_time

      tw_start, tw_end = solution.problem_data['time_window'][tour[idx]]
      if current_time > tw_end:
        return False

      # Add the service time for the current node after arriving and waiting
      current_time += solution.problem_data['service_time'][tour[idx]]

  return True

==> Base-model/vio_temp.tex <==
def calculate_violation_score(solution: VrpState) -> float:
  """
  Args:
    solution (VrpState): An object representing the VRP solution.
      - problem_data (dict): A dictionary with problem details; Use only defined values in "Check Constraints Code".
      - routes (list): A list of routes, where each route is a list of node IDs (integers, excluding the depot).
      - cost (Callable[[], float]): Implemented method to compute and return the total cost of the solution's routes.
  Returns:
    violation_score (float): The calculated constraint violation score, where higher scores indicate more severe violations.

  Note:
    Do not use data or methods that is not contained in the "solution" object.
  """
  # Your code goes here ...

